Plug it and Play on Logs: A Configuration-Free Statistic-Based Log Parser

Log parsing is an essential task in log analysis, and many tools have been designed to accomplish it. Existing log parsers can be categorized into statistic-based and semantic-based approaches. In comparison to semantic-based parsers, existing statistic-based parsers tend to be more efficient, require lower computational costs, and be more privacy-preserving thanks to on-premise deployment, but often fall short in their accuracy (e.g., grouping or parsing accuracy) and generalizability. Therefore, it became a common belief that statistic-based parsers cannot be as effective as semantic-based parsers since the latter could take advantage of external knowledge supported by pretrained language models. Our work, however, challenges this belief with a novel statistic-based parser, PIPLUP. PIPLUP eliminates the pre-assumption of the position of constant tokens for log grouping and relies on data-insensitive parameters to overcome the generalizability challenge, allowing "plug and play" on given log files. According to our experiments on an open-sourced large log dataset, PIPLUP shows promising accuracy and generalizability with the data-insensitive default parameter set. PIPLUP not only outperforms the state-of-the-art statistic-based log parsers, Drain and its variants, but also obtains a competitive performance compared to the best unsupervised semantic-based log parser (i.e., LUNAR). Further, PIPLUP exhibits low time consumption without GPU acceleration and external API usage; our simple, efficient, and effective approach makes it more practical in real-world adoptions, especially when costs and privacy are of major concerns.

==> sections/removed_contents.tex <==
\noindent\underline{\textbf{Evaluating the impact of $K$}}. $K$ determines the number of entries on the frequent tokens layer. To understand the impact of $K$ on the parsing performance and verify our assumption about $K$'s global insensitivity, we evaluate PIPLUP with $K =\{5,10,15,20\}$. %, and the $\theta_{br}$ is fixed to 2 to control the variable. 
According to Table~\ref{tab:rq1}, PIPLUP's parsing performance on the same dataset is not sensitive to the change of $K$: on average, the gap between the best and worst performance values is below 1\% for all four metrics. The same pattern applies to individual datasets: on 9 out of the 10 datasets, the gap between the best and worst performance in terms of all four metrics is below 1\%. The only exceptions are Linux and HealthApp, where $K=10$ slightly clustered the logs better. The default setting ($K$=15) achieves the best performance for 8 out of the 10 datasets. 
\textbf{Our evaluation confirms our assumption that $K$ is a \emph{globally insensitive} parameter.}


\subsubsection{\textbf{\underline{Statistical Frequent Token Bag Construction}}}
%\heng{maybe call it statistical or approximate frequent token bag construction, to highlight the novelty for better efficiency?}
\label{sec:tree_step2}
After preprocessing, we tokenize the log messages with blank spaces. Previous research showed that log messages sharing the same frequent tokens tend to share the same template~\citep{jiang2024lilac, jiang2024large,nagappan2010abstracting}. Therefore, it is effective to use frequent tokens for log clustering. Jiang \textit{et al.}~\citep{jiang2024lilac} tokenized each log message and calculated the token frequencies. The top-$K$ most frequent tokens in the full dataset are selected as the coarse feature of a log message and are used for clustering at the initial step. Although this procedure is effective for log clustering, detecting the most frequent tokens on an overall scale requires a great amount of time: Jiang \textit{et al.} mentioned that the time overhead of LILAC is majorly caused by the clustering process, posing a critical issue in processing large log files. %\heng{earlier this paragraph only mentions ``clustering'': keep it consistent}

Hence, we take an alternative strategy to suppress the time overhead by creating a frequent token bag using a log subset. To ensure the subset has captured the majority of the frequent tokens, the size of the subset should represent the log lines on at least a 95\% confidence level with a 5\% error margin. The sampled logs are then split into tokens, and distinct token entries will be ranked in decreasing order of their frequencies. Afterward, the $K$ tokens with the highest frequencies are selected to create a \textit{frequent token bag}. 

Although many variables can be identified and converted into placeholders in the preprocessing stage~\citep{qin2025preprocessing}, there are still variables without generalizable patterns (e.g., ``syslogd'' in message ``syslogd startup succeeded'') in the preprocessed log message. Therefore, we cannot directly identify the constants at the first occurrence of a message: if a log message cannot match with any existing log clusters, it will be stored under a default ``None'' node, indicating that its constant is unknown. 

The log messages would be represented by the most frequent token in the \textit{frequent token bag} on the \textbf{Frequent Token Level}%\xingfang{``level'' is more commonly used in tree structure.}
, because they have higher chances to be constant tokens, according to the frequency heuristics~\citep{dai2020logram, vaarandi2003data, nagappan2010abstracting, vaarandi2015logcluster}. For example, assume two tokens ``node'' and ``bytes'' are among the top $K$ tokens, and ``bytes'' has a frequency of 100, while the frequency of ``node'' is only 10. Assume a log message contains both these two frequent tokens, its internal node on the frequent token layer should be ``bytes'' since the token is the most frequent one the log message has. On the other hand, we may also encounter log messages matching with no frequent tokens. In this circumstance, the log message %\xingfang{Not sure if I am correct, less frequent tokens seem to be more distinctive?}

\noindent\textbf{Case 1: Token is in the token list.} In the first case, the token of the incoming log message exists in the token list. We append the token to the new path list and ``False'' to the update flag list, since no information update is detected at this position. 

\noindent\textbf{Case 2: Token is not in the token list, and the list length is below $\theta_{br}$.} Given the list length is below the threshold, we regard the new token as a constant. We append the token to the token list and the new path list, then add ``True'' to the update flag list, since a new constant is added to the token list at this position. 

\noindent\textbf{Case 3: Token is not in the token list, and the list length equals $\theta_{br}$.} Given that adding the new token will make the list exceed the branching threshold, the tokens in this position for all templates shall be converted to a variable placeholder. In this case, we update all existing templates in the cluster, append the placeholder to the token list and the new path list, and add ``True'' to the update flag list, since this token triggered a global change in cluster templates.

\noindent\textbf{Case 4: Token is not in the token list, and the list length equals $\theta_{br}$.} If case 3 is triggered, then all the incoming log messages shall have a variable placeholder at the corresponding position. Therefore, we directly append the placeholder to the new path list and add ``False'' to the update flag list.

PIPLUP compares the token at each position with the corresponding list in the token bag. For instance, the first token in the log message will be compared against the list for ``T1'' in the token bag. We also leverage an update flag list to denote the change in cluster information, and a new path to document the resulting token list from the incoming message. The comparison could fall into four mutually exclusive cases, which require different handling methods listed in Table~\ref{tab:branch_cases}: 

\noindent\textbf{Case 1: Token is in the token list.} 

\noindent\textbf{Case 2: Token is not in the token list, and the list length is below $\theta_{br}$.} 

\noindent\textbf{Case 3: Token is not in the token list, and the list length equals $\theta_{br}$.} 

\noindent\textbf{Case 4: Token is not in the token list, and the list length equals $\theta_{br}$.} 

\input{tables/case_handling}

After scanning through the log message, we check whether the message brings any information update (i.e., a ``True'' in the update flag list). If the message updates cluster information, we append the new path to the path list and 

==> tables/case_handling.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The handling methods for the four comparison cases at sequence position $i$. ``-'' indicates no action required. }
\label{tab:case_handling}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Case}   & \textbf{NewPath} & \textbf{TokenBag[$T_i$]} & \textbf{PathList}                 & \textbf{UpdateFlagList} \\ \hline
\textbf{Case 1} & +token & -      & - & +False \\ \hline
\textbf{Case 2} & +token & +token & - & +True  \\ \hline
\textbf{Case 3} & +\textless*\textgreater             & +token               & for path in PathList, path[i]=\textless*\textgreater & +True                   \\ \hline
\textbf{Case 4} & +\textless*\textgreater   & -      & - & +False \\ \hline
\end{tabular}%
}
\end{table}

==> tables/different_K.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The average parsing efficiency and effectiveness of PIPLUP with different choices of the $K$ value.}
\label{tab:different_K}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{K} & \textbf{Time} & \textbf{GA}    & \textbf{PA}    & \textbf{FGA}   & \textbf{FTA}   \\ \hline
5          & 11.558        & 0.916          & \textbf{0.767}          & 0.900          & 0.716          \\ \hline
10         & 11.644        & 0.916          & \textbf{0.767}          & 0.901          & \textbf{0.717}          \\ \hline
15         & 11.591        & \textbf{0.917} & \textbf{0.767} & \textbf{0.902} & \textbf{0.717} \\ \hline
20         & 11.458        & \textbf{0.917} & \textbf{0.767} & \textbf{0.902} & \textbf{0.717} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/different_br_thresh.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The average parsing efficiency and effectiveness of PIPLUP with different choices of the $\theta_{br}$ value.}
\label{tab:different_br_thresh}
\resizebox{0.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{$\theta_{br}$} & \textbf{Time} & \textbf{GA}    & \textbf{PA}    & \textbf{FGA}   & \textbf{FTA}   \\ \hline
1         & 10.851        & 0.898          & 0.732          & 0.827          & 0.655          \\ \hline
2          & 11.591        & \textbf{0.917} & \textbf{0.767} & \textbf{0.902} & \textbf{0.717} \\ \hline

\end{tabular}%
}
\end{table}

%3          & 12.265        & 0.895          & 0.760          & 0.877          & 0.702          \\ \hline
%4          & 14.188        & 0.898          & 0.765          & 0.874          & 0.702          \\ \hline

==> tables/different_sim_thresh.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{The average parsing efficiency and effectiveness of PIPLUP with different choices of the $\theta_{sim}$ value.}
\label{tab:different_sim_thresh}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{$\theta_{sim}$} & \textbf{Time} & \textbf{GA}    & \textbf{PA}    & \textbf{FGA}   & \textbf{FTA}   \\ \hline
0.4 & 23.959 & 0.849 & 0.721 & 0.845 & 0.650 \\ \hline
0.5 & 10.027 & 0.897 & 0.751 & 0.869 & 0.687 \\ \hline
0.6 & 49.805 & 0.899 & 0.761 & 0.826 & 0.665 \\ \hline
0.7 & 92.719 & 0.898 & 0.737 & 0.746 & 0.603 \\ \hline
default                & 11.591        & \textbf{0.917} & \textbf{0.767} & \textbf{0.902} & \textbf{0.717} \\ \hline
\end{tabular}%
}
\end{table}

==> tables/parsing_example.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{An example of log parsing.}
\vspace{-1mm}
\label{tab:variable_extraction}
%\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{l|l  }
\hline
\textbf{Log Message}   & creating device node `/udev/vcs7'                                             \\ \hline
\textbf{Template}  & creating device node \textless*\textgreater \\ \hline
\textbf{Variables} & `/udev/vcs7'                                                                                   \\ \hline
\end{tabular}%
%}
\vspace{-3mm}
\end{table}
